Combining Peer-to-Peer and Cloud Computing for Large Scale On-line Games

This thesis investigates the combination of Peer-to-Peer (P2P) and Cloud Computing to support Massively Multiplayer On- line Games (MMOGs). MMOGs are large-scale distributed applications where a large number of users concurrently share a real-time virtual environment. Commercial MMOG infrastructures are sized to support peak loads, incurring in high economical cost. Cloud Computing represents an attractive solution, as it lifts MMOG operators from the burden of buying and maintaining hardware, while offering the illusion of infinite machines. However, it requires balancing the tradeoff between resource provisioning and operational costs. P2P- based solutions present several advantages, including the inherent scalability, self-repairing, and natural load distribution capabilities. They require additional mechanisms to suit the requirements of a MMOG, such as backup solutions to cope with peer unreliability and heterogeneity. We propose mechanisms that integrate P2P and Cloud Computing combining their advantages. Our techniques allow operators to select the ideal tradeoff between performance and economical costs. Using realistic workloads, we show that hybrid infrastructures can reduce the economical effort of the operator, while offering a level of service comparable with centralized architectures.

==> frontmatter/dedication.tex <==
% Alessio Botta 2008 - alebotta@gmail.com
%
% phdimt class file and demo
% A LaTex implementation of IMT Lucca PhD Thesis style
% Please send an email to let me know you used this style.

\begin{dedication} 
To Mileva
\end{dedication}

==> mainmatter/workload.tex <==


%\chapter{Workload}

The management of a MMOG infrastructure generates a certain amount of load on the server, in terms of computational and bandwidth requirements.
A realistic simulation of the load is central to properly evaluate a MMOG infrastructure.
This thesis focuses on one type on load, which is bandwidth.
In particular, the outgoing bandwidth is considered.
This is done for the following reasons.
First, besides machine time, a typical on-demand computing platform charges outgoing bandwidth.
Hence, with the reduction of the outgoing bandwidth it is possible to reduce the operational costs of the infrastructure.
Second, user-provided resources usually have asymmetric connections to the public network.
This implies that the outgoing bandwidth is the resource to optimize, due to the smaller availability compared to the ingoing bandwidth. 
%
In addition, our workload considers the load related to the management of the users. It does not take into account the bandwidth consumed for other tasks, like backup management, intra-server communications, and other services at application level (e.g. voice over IP).  
In the rest of the chapter the generic term load is used to indicate the outgoing bandwidth load.



Mostly, the load depends on the number of concurrent players connected to the infrastructure.
For instance, \cite{Nae2008} noticed that the load varies from $O(n)$ to $O(n^3)$ according to the pace of interaction provided by the particular MMOG (where $n$ is the number of players). However, a wide analysis is necessary to reproduce the peculiarities of a proper MMOG load. At this regard, we have considered the following aspects when building a synthetic workload for MMOGs: (i) the variation in the number players over time, (ii) the players’ mobility patterns, (iii) the objects distribution, and (iv) the interaction model.




\paragraph{Interaction model}

In our model bandwidth is sampled according to a discrete time step model.
We define each step $t$ to have a duration of $\Delta t$.
During the step duration, for each generic entity $e$ the server gathers all the state actions regarding $e$.
Then, a new state is computed and it is broadcast to the interested players, i.e. the players that have the $e$ in their AOI.
This broadcasting is the action that consumes outgoing bandwidth. Hence, the bandwidth requirement at a generic time $t$ is computed with the formula:

\begin{equation}
\sum_{e \in E}{e_{AOI}(t)} \times M_{len}
\end{equation} 


\noindent
where $E$ is the set of all entities. $M_{len}$ is the length of the broadcast message, which we assume to be the same for any entity.
$e_{AOI}(t)$ is the number of AOI's in which the entity $e$ is at time $t$. This value has been defined experimentally, through the simulation of players’ movements and objects placement in the virtual world.




\paragraph{Number of Players}

The number of concurrent players connected to a MMOG infrastructure presents seasonal trends. These trends can regard period of the week (i.e. more players in the weekend rather than in the middle of the week) and period of the day (i.e. more player in the evening rather than in the morning). In any case, it is a central point to evaluate how a MMOG infrastructure adapts itself to these variations. In particular, since the load is in a direct correspondence with the number of players, we are interested in the impact of a variable number of players on the infrastructure.


In order to simulate a seasonal trend in our workload, we vary the number of players over the time. To compute the number of players at a given time $t$ we use the following formula:

\begin{equation}
\sin(\frac{\pi t}{\lambda}) \times P_{max}
\end{equation}

\noindent
where the variation is controlled by two parameters: (i) the maximum number of player $P_{max}$ and (ii) the length $\lambda$, which represents the number of iteration that are needed to perform a season cycle. 


\paragraph{Players Mobility Model}

Avatars move on the map according to realistic mobility traces that have been computed according the mobility model presented by Legtchenko et al.  \cite{Legtchenko2010},  which simulates avatars movement in a commercial MMOG, Second Life \cite{sl-site}.
We have presented this implementation in \cite{carlini2011evaluating}, as well as a comparison with other mobility models.
%
In the model, players gather around a set of {\em hotspots}, which usually correspond to towns, or in general to points of interest of the virtual world. A circular area characterized by a center and by a radius defines each hotspot.
Traces generation goes through two phases: \textit{initialization} and \textit{running}.



In the initialization phases, the area of the of the virtual environment is divided in \textit{hotspot area} and \textit{outland area}. The percentage of the hotspot area is defined by $p_{hot}$ and, consequently $1 - p_{hot}$ represents the outland area.
The hotspots are placed randomly in the virtual environment. The number of hotspot is defined by the parameter $H_{num}$. Their radius is computed such that the total area covered by the hotspots is in accordance to $p_{hot}$.
The parameter $p_{den}$ defines the probability that a player would be initially placed in an hotspot, whereas $1 - p_{den}$ defines the probability for a player to be initially placed in outland. 
If the player is placed in the outland, its position is chosen uniformly at random on the whole map.
Otherwise, an hotspot for the player is randomly selected and the player is positioned inside the hotspot.
The position inside the hotspot is chosen by considering a Zipfian\footnote{The Zipfian distribution was originally studied to show the relation of inverse proportionality between the frequency of words in a text and their rank in the frequency table. Nowadays, it used in many field of computer science, like graph theory \cite{broder2000graph},  to model similar concepts. In our work we use this distribution to model the fact that the frequency of entities is inversely proportional to their distance from the center of the hotspot.} distribution \cite{newman2005power}, so to ensure an higher density of players near the center of the hotspot.


The running phase moves the players across the virtual environment. The movements are driven by a Markov chain, whose transition probabilities are taken from the original paper \cite{Legtchenko2010}. The possible states for the players are the following: 

\begin{itemize}
\item \textit{Halt}(H): the player remains in place.
\item \textit{Exploration}(E): the player explores a specific area. If the player is moving inside an hotspot, the new position is chosen according to a power law distribution. Otherwise, the new position is chosen at random.
\item \textit{Travelling}(T): the player moves straight toward another point in the virtual environment. The new point is chosen in accordance with $p_{dens}$.
\end{itemize}

Initially every player is in state H. At each step $t$, the model decides the new state according to the probability of moving between states.
This mobility model exposes a fair balance between the time spent by avatars in hotspots and outland. 
Furthermore, the path followed by avatars when moving between hotspots is not static, 
i.e. no predefined path connects two hotspots. 


\paragraph{Objects distribution}

Like players movement, the distribution of the objects exploits the concept of hotspots.
The idea is to have more objects in the hotspots, which represent a place of interest in the virtual world.
To place objects over the virtual environment, we use the same space characterization in desert and hotspot areas used by the mobility model. 
The total number of objects is defined as $O_{num}$. A  fraction of these objects is placed inside hotspot areas, whereas the rest is placed in the desert area.
%
The percentage of objects that are placed inside the hotspot area is controlled by the parameter $p_{obj}$. Objects in an hotspot area are placed so that their concentration follows a Zipfian distribution \cite{newman2005power}, with a peak in the hotspot center. Conversely, objects in the desert area are placed randomly.\\


%Objects inside hotspots are characterized by a popularity, modelling the probability of an interaction between that
%object and a player. Object's popularity is assigned according to a power law distribution, each value computed regardless of the object's position inside the hotspot. The remaining 35\% of the objects lay in the outland area and it is distributed 
%according to a uniform random distribution, and their popularity is fixed to a constant value (1 in the experiments). 


\begin{table}
\centering
\begin{tabular}{|c|c||c|c|}
\hline
$M_{len}$ & 100 bytes & $\lambda$ & 200 \\
\hline
$P_{max}$ & 1000 & $O_{num}$ & 1000 \\
\hline
$P_{obj}$ & 0.7 & $H_{num}$ & 5 \\
\hline
$p_{den}$ & 0.8 & $p_{hot}$ & 0.3 \\
\hline
size & 5000x5000 & $\Delta t$ & 0.2s \\
\hline
\end{tabular}
\caption{Workload's table of parameters}\label{tab:par-work}
\end{table}

Figure \ref{fig:obj-place} shows the placement of 5000 objects in a virtual environment characterized by the parameters in Table \ref{tab:par-work}.


\begin{figure}
\centering
        \begin{subfigure}[b]{0.45\textwidth}
                \centering
                \includegraphics[width=\textwidth]{images/ds1}
                \caption{Load variation with number of player over time}
                \label{fig:dataset}
        \end{subfigure}%
        \quad      
        \begin{subfigure}[b]{0.45\textwidth}
                \centering
                \includegraphics[width=\textwidth]{images/heat2}
                \caption{Objects placement in the virtual environment area}
                \label{fig:obj-place}
        \end{subfigure}%
\caption{Workload characterization}\label{fig:dset-char}
\end{figure}


